Learning to Fuse 2D and 3D Image Cues for Monocular Body Pose Estimation

Most recent approaches to monocular 3D human pose estimation rely on Deep Learning. They typically involve regressing from an image to either 3D joint coordinates directly or 2D joint locations from which 3D coordinates are inferred. Both approaches have their strengths and weaknesses and we therefore propose a novel architecture designed to deliver the best of both worlds by performing both simultaneously and fusing the information along the way. At the heart of our framework is a trainable fusion scheme that learns how to fuse the information optimally instead of being hand-designed. This yields significant improvements upon the state-of-the-art on standard 3D human pose estimation benchmarks.

==> figs/approach.tex <==
% !TEX root = ../top.tex

\begin{figure*}
	\def\tabularxcolumn#1{m{#1}}
	\begin{tabularx}{\linewidth}{@{}Xc@{}}
		%
		\subfloat[Trainable Fusion]{\includegraphics[width=\columnwidth, height=8cm]{trainable_fusion.pdf}}
		&
		\begin{tabular}{c}
			\subfloat[Early Fusion]{\includegraphics[width=\columnwidth]{early_fusion_iccv.png}} \\    
			\subfloat[Late Fusion]{\includegraphics[width=\columnwidth]{late_fusion_iccv.png}}    
		\end{tabular}

	\end{tabularx}
	
	\caption{{\bf Three different instances of our general fusion framework.}
		The  three different  fusion strategies  depicted here  all follow  the
		pattern  shown in  Fig.~\ref{fig:intro}.  \pf{  They combine  2D joint
			location probability maps  with 3D cues directly  extracted from the
			input  image.}  In  these  four  networks,  we  denote  by  $C$  the
		convolutional layers and by $FC$ the fully-connected ones. The numbers
		below each layer  represent the corresponding size of  the feature map
		for convolutional layers and the number of neurons for fully connected
		ones.}
	\label{fig:architecture}
\end{figure*}

